Maximum Weight Online Matching with Deadlines

We study the problem of matching agents who arrive at a marketplace over time and leave after d time periods. Agents can only be matched while they are present in the marketplace. Each pair of agents can yield a different match value, and the planner's goal is to maximize the total value over a finite time horizon. First we study the case in which vertices arrive in an adversarial order. We provide a randomized 0.25-competitive algorithm building on a result by Feldman et al. (2009) and Lehman et al. (2006). We extend the model to the case in which departure times are drawn independently from a distribution with non-decreasing hazard rate, for which we establish a 1/8-competitive algorithm. When the arrival order is chosen uniformly at random, we show that a batching algorithm, which computes a maximum-weighted matching every (d+1) periods, is 0.279-competitive.

==> algorithm_ro.tex <==
% !TEX root = adv_paper.tex

\section{The Batching Algorithm}

The batching algorithm computes a maximum-weight matching every $d$ time steps. It then matches every vertex in the matching. Unmatched vertices are discarded.

In many practical cases, dynamic matching is done through a variation of Batching. In the context of Kidney Exchange for example, most programs operate on a fixed schedule (every day, week, month, etc). In the context of car-pooling, platforms periodically compute a maximum-weight matching to dynamically match passengers with each other.

In this context, the adversarial scenario seems very pessimistic. We make the assumption that the adversary chooses the graph structure, but not the arrival order, which is similar to assuming that the adversary chooses a distribution of arrivals which is unknown to the online algorithm.

The purpose of this section is two-fold. First we wish to provide theoretical garantees on the performance of Batching when vertices arrive in random order. Second, we improve on the best known bound of $1/4$ for the Fully Online Matching problem with edge-weighted graphs under random order arrivals.

% Let us define the offline algorithm, for simplicity, suppose that the time horizon $T$ is a multiple of $d$ and that $d$ is an even number. Conditional on $\v$, the offline matching solves the following LP:
% \begin{equation}
% \begin{split}
% \off(\v) = \max &\sum_{i = 1}^{T} \sum_{j = i}^{i+d} x_{i,j} w_{i,j}(\v) \\
% \text{s.t.} &\sum_j x_{i,j} \leq 1 \text{   } \forall i \in \mathbb{[} 1, K \mathbb{]} \\
% &x_{i,j} \in \{0,1\}
% \end{split}
% \label{eq:MIP}
% \end{equation}
% Where we have $w_{i,i} = 0$ for all $i$.
% Let $x^*$ be a solution to \eqref{eq:MIP},
% %We consider a simplified model where each node stays exactly $d$ time steps after arriving. In other words we set $w_{i,j} = 0$ when $\mid i - j \mid > d$.
%
% Let us now consider a batching algorithm $\bat$ which conducts a maximum weight matching every $d$ time steps, and discards any unmatched nodes. Conditional on an arrival sequence $\v = v_1, v_2, ... v_T$, every $d$ time steps, $\bat$ solves:
% \begin{equation}
% \begin{split}
% \bat_s(\v) = \max &\sum_{i = sd+1}^{(s+1)d} \sum_{j = i+1}^{(s+1)d} x_{i,j} w_{i,j}(\v) \\
% \text{s.t.} &\sum_j x_{i,j} \leq 1 \text{   } \forall i \in T \\
% &x_{i,j} \in \{0,1\}
% \end{split}
% \label{eq:MIP_batch}
% \end{equation}
% And the total reward is $\bat = \sum_{s = 1}^{T/d} \bat_s$.
%
\begin{theorem}
  \label{th:competitive_ratio}
Batching is $0.279$-competitive.
\end{theorem}
%
% \begin{proof}
% The idea of the proof is as follows: under OFF, a vertex that arrives at time $i$ has opportunities to match to vertices arrived between $i - d$ and $i + d$, therefore we can find 4 arrival sequences such that BAT has the opportunity to match any nodes that OFF matches.


==> analysis.tex <==
% !TEX root = adv_paper.tex

\section{Alternative algorithm: Dynamic Deferred Acceptance}
\label{sec:analysis}
In this section, we prove our three main results. We use $\mathcal{A}$ to denote the expected sum of all match values collected by the algorithm, and $\mathcal{O}$ to denote the value of the offline maximum-weight matching.

\subsection{Proof of Proposition \ref{prop:factor2}}

We  prove that \emph{DDA} (Algorithm 1) obtains a competitive ratio of at least $\nicefrac{1}{2}$ on constrained bipartite graphs.  The proof follows the primal-dual framework.

First, we observe that by complementary slackness, any seller $s$ (buyer $b$) that departs unmatched has a final price $p_s^f = 0$ (final profit margin $q_b^f = 0$). When a seller $s$ is critical and matches to $b$, we have  $v_{s,b} = p_s^f + q_b^f$. Therefore, \emph{DDA} collects a reward of $\mathcal{A} = \sum_{s \in S} p_s^f + \sum_{b \in B} q_b^f$.

Second, let us consider a buyer $b$ and a seller $s \in [b - d, b)$ who has arrived before $b$ but not more than $d$ steps before. Because sellers do not finalize their matching before they are critical, we know that $s \in S_b$. An ascending auction may be triggered at the time of $b$'s arrival, after which we have: $v_{s,b} \leq p_s(b) + q_b(b) \leq p_s^f + q_{b}^i$, where the second inequality follows from the definition that $q_b(b) = q_b^i$ and from the monotonicity of sellers' prices (Lemma \ref{lem:mon}). Thus, $(p^f, q^i)$ is a feasible solution to the offline dual problem.

Finally, we observe that upon the arrival of a new buyer, the ascending auction does not change the sum of prices and margins for vertices who were already present:

\begin{claim}
  \label{cl:monotonicity}
  Let $b$ be a new buyer in the market, and let $p, q$ be the prices and margins before $b$ arrived, and let $S_t$ and $B_t$ be the set of sellers and buyers present before $b$ arrived. Let $p'$, $q'$ be the prices and margins at the end of the ascending auction phase (Step 2(a) in Algorithm 1). Then:
\begin{equation}
\sum_{s \in S_t} p_s + \sum_{b \in B_t} q_b = \sum_{s \in S_t} p'_s + \sum_{b \in B_t} q'_b.
\label{eq:conservation}
\end{equation}
\end{claim}
The proof of Claim \ref{cl:monotonicity} is deferred to Appendix \ref{app:missing_proofs}.
By applying this equality iteratively after each arrival, we can relate the initial margins $q^i$ to the final margins $q^f$ and prices $p^f$:
\begin{claim}
  \label{cl:conservation}
  $\sum_{s \in S} p_s^f + \sum_{b \in B} q_b^f = \sum_{b \in B} q_b^i$.
\end{claim}

This completes the proof of Proposition \ref{prop:factor2} given that the offline algorithm achieves at most:
$$\mathcal{O} \leq \sum_{s \in S} p_s^f + \sum_{b \in B} q_b^i \leq 2 \mathcal{A}.$$

It remains to prove Claim \ref{cl:conservation}.

\begin{proof}[Proof of Claim \ref{cl:conservation}]
The idea of the proof is to iteratively apply the result of Claim \ref{cl:monotonicity} after any new arrival.
Let $\widetilde{S}_t$ (resp. $\widetilde{B}_t$) be the set of sellers (buyers) who have departed, or already been matched before time $t$. We show by induction over $t \leq T$ that:

\begin{equation}
  \sum_{s \in \widetilde{S}_t} p_s^f + \sum_{b \in \widetilde{B}_t} q_b^f + \sum_{s \in S_t} p_s(t) +  \sum_{b \in B_t} q_b(t) = \sum_{b \in \widetilde{B}_t} q_b^i +  \sum_{b \in  B_t} q_b^i.
  \label{eq:proof:balance}
\end{equation}
This is obvious for $t = 1$. Suppose that it is true for $t \in [1, T-1]$. Note that departures do not affect \eqref{eq:proof:balance}. If the agent arrivint at $t + 1$ is a seller, then for all other sellers $s$, $p_s(t+1) = p_s(t)$ and for all buyers $b$, $q_b(t+1) = q_b(t)$, thus \eqref{eq:proof:balance}, is clearly still satisfied. Suppose that vertex $t + 1$ is a buyer. Using equation \eqref{eq:conservation}, we have:

$$\sum_{s \in S_{t+1}} p_s(t+1) +  \sum_{b \in B_{t+1}} q_b(t+1) = q_{t+1}(t+1) + \sum_{b \in B_t} q_b(t) + \sum_{s \in S_t} p_s(t) = \sum_{b \in  B_{t+1}} q_b^i.$$

Note that at time $T + d$, every vertex has departed. Thus, $\widetilde{S}_{T+d} = S$, $\widetilde{B}_{T+d} = B$ and $S_{T+d} = B_{T+d} = \emptyset$.
This enables us to conclude our induction and the proof for \eqref{eq:proof:balance}.

\end{proof}

\subsection{Proof of Corollary \ref{cor:factor8}}

We  prove  that \emph{SDDA} is $\nicefrac{1}{8}$-competitive for
arbitrary graphs.

The Offline algorithm solves the following maximum-weight matching problem:

  \begin{equation}
  \begin{split}
  \mathcal{O} = \max & \sum_{k < l \in [1, T]} v_{k, l} x_{k, l} \\
  \text{ s.t. } &\sum_{k < l} x_{k,l} + \sum_{k > l} x_{l, k} \leq 1 \\
   & x_{k,l} \in \{0, 1\}. \\
  \end{split}
  \label{eq:offline:primal}
  \tag{Offline Primal}
  \end{equation}

  Suppose that we have assigned each vertex $k \in [1,T]$ to be either a buyer or a seller with probability $1/2$. For $k < l$, let $\widetilde{v}_{k,l} = v_{k,l} \mathds{1}_{k \in S, l \in B}$.
  Consider the \emph{constrained} offline problem obtained by running \eqref{eq:offline:primal} with edge values $\tilde{v}$. Its expected reward is at least $\nicefrac{1}{4}$ of the offline reward $\mathcal{O}$: Let $x^*$ be an optimal solution to equation \eqref{eq:offline:primal}. It is feasible for the \emph{constrained} problem, and yields value equal to $\mathbb{E}\left[\sum_{k < l \in [1, T]} v_{k,l} x^*_{k,l} \mathds{1}_{k \in S, l \in B} \right] = \frac{1}{4} \mathcal{O}$.

  We can conclude using Claim \ref{cl:conservation} along with the fact that $(p_s^f)_{s \in S}, (q_b^i)_{b \in B}$ is a feasible solution to the constrained offline dual problem.
  This yields the \nicefrac{1}{8} competitive ratio. \qedsymbol

\subsection{Proof of Theorem \ref{th:factor4}}

We   prove that the PDDA algorithm achieves a competitive ratio of at least $\nicefrac{1}{4}$ for  arbitrary graphs.
Observe that because of the randomization, we collect in expectation
$$\mathcal{A} = \E\left[\sum_{t \text{ is a seller}} p_{s_t}^f + \sum_{t \text{ is a buyer}} q_{b_l}^f\right] = \frac{1}{2} \sum_{t \in [1, T]} p_{s_t}^f + q_{b_t}^f.$$

Using the convention that for a pair of vertices $k,l$, $v_{k,l} = 0$ when $|k - l| > d$, the dual of the offline matching problem linear programs can be written as:

\begin{equation}
\begin{split}
\min & \sum_{k \in [1,T]} \lambda_k\\
\text{s.t. } & v_{k,l} \leq \lambda_k + \lambda_l \\ %\text{, } \forall k < l \leq k+d \\
& \lambda_k \geq 0.
\end{split}
\label{eq:offline:dual}
\tag{Offline Dual}
\end{equation}


It is enough to show that $(p_{s_k}^f + q_{b_k}^i)_{k \in [1, T]}$ is a feasible solution to equation \eqref{eq:offline:dual}.
This is similar to the proof in the simplified setting. Fix $(k, l) \in [1, T]^2$ and assume that $k < l \leq k + d$. When $l$ arrives, we have $s_k \in S(l)$, therefore $v_{k,l} \leq p_{s_k}(l) + q_{b_l}^i$ by dual feasibility during the online matching procedure. Using the Lemma \ref{lem:mon}, we get feasibility for equation \eqref{eq:offline:dual}:
$$ p_{s_k}^f + q_{b_k}^i + p_{s_l}^f + q_{b_l}^i \geq v_{k,l}.$$

We can conclude the factor $4$ using Claim \ref{cl:conservation}.   \qedsymbol


==> hardness.tex <==
% !TEX root = adv_paper.tex


\section{Adversarial Arrival Order: relaxing departure assumptions}
\label{sec:hardness}

Here we show that no algorithm is constant-competitive in the case where we let departures be chosen by an adversary, or if the departures are stochastic and the algorithm does not know when vertices become critical.

% \subsection*{Upper Bounds}
% \begin{claim}
% No deterministic algorithm is constant-competitive, and no randomized algorithm is more than $\nicefrac{1}{2}$-competitive.
% \end{claim}
% \begin{proof}
% 	Observe that in Figure \ref{fig:hard:basic},
% \end{proof}

We consider the \emph{Adversarial departures} (AD) setting, where the adversary is allowed to choose the departure time $d_i$ of vertex $i$. We assume that the online algorithm knows $d_i$ at the time of arrival of $i$.

\begin{claim}
No algorithm is constant-competitive in the AD setting.
\end{claim}
\begin{proof}
  Let us consider a graph $G_K$ with $n$ vertices, where $K$ will be chosen later by the adversary. For all $j \in [2,K]$, $v_{1,j} = M^j$, and for all other $(i,j)$, $v_{i,j} = 0$. Assume that vertex $1$ departs after $n$ arrivals, while all other vertices depart right away. For $k \geq 2$, let $x_k$ be the probability that the online algorithm matches vertex $1$ to $k$ when $k$ arrives.
  Observe that because the algorithm does not know $K$, the $x$ has to be valid when $K = n$. Therefore, $\sum_{k = 1}^n x_k \leq 1$.
  Therefore, there exists $k$ such that $x_k \leq 1/n$. The adversary chooses $K = k$. This implies that $\A = \sum_{j \leq k} x_j M^j \leq \frac{M^k}{n} + M^{k-1} \leq \frac{2}{n} \mathcal{O}$, where the last inequality is obtained by taking $M \geq n$.
\end{proof}

\begin{figure}[!ht]
  \centering
  \begin{tikzpicture}[pre/.style={<-,shorten <=1.5pt,>=stealth,thick}, post/.style={->,shorten >=1pt,>=stealth,thick}, scale=0.7]
    \tikzstyle{every node}=[draw,shape=rectangle,minimum size=5mm, inner sep=0];
    \tikzstyle{edge} = [draw,thick,-]
    \tikzstyle{every node}=[shape=circle,minimum size=8mm, inner sep=0];

    \draw [fill](-14,0) circle [radius=0.2];
    \node [right] at (-14.7,-0.8) {$1$};
    \draw [fill](-12,0) circle [radius=0.2];
    \node [right] at (-12.7,-0.8) {$2$};
    \node [right] at (-13.2, 0.3) {$1$};
    \draw[line width=1.5pt] [-] (-14+0.25, 0) .. controls(-13,0) ..(-12-0.25, 0);

    \draw [fill](-10,0) circle [radius=0.2];
    \node [right] at (-10.7,-0.8) {$3$};
    \node [right] at (-11.3,0.9) {$M$};
    \draw[line width=1.5pt] [-] (-14+0.25, 0.25) .. controls(-12,1) ..(-10-0.25, 0.25);

    \draw [fill](-8,0) circle [radius=0.2];
    \node [right] at (-8.7,-0.8) {$...$};
    \draw[line width=1.5pt] [-] (-14+0.25, 0.25) .. controls(-11,2) ..(-8-0.25, 0.25);

    \draw [fill](-6,0) circle [radius=0.2];
    \node [right] at (-6.7,-0.8) {$K$};
    \node [right] at (-9,2.5) {$M^K$};
    \draw[line width=1.5pt] [-] (-14+0.25, 0.25) .. controls(-10,3) ..(-6-0.25, 0.25);

    \draw [fill](-4,0) circle [radius=0.2];
    \node [right] at (-4.7,-0.8) {$K+1$};
    \draw [fill](-2,0) circle [radius=0.2];
    \node [right] at (-2.7,-0.8) {$...$};

  \end{tikzpicture}
    \caption{Graph where $d_1 = N$ and $d_i = 0$ for all $i > 1$. Vertices $k > K$ have no edges.}
  \label{fig:adv_dep}
\end{figure}

We now consider the \emph{Adversarial departure distribution} (ADD) setting where $d_i$ are sampled i.i.d from a distribution chosen by the adversary. We assume furthermore that the online algorithm knows the realization $d_i$ upon the arrival of vertex $i$.

\begin{claim}
No algorithm is constant-competitive in the ADD setting
\end{claim}
\begin{proof}
  The idea is that we can construct a graph that exhibits the same properties as Figure \ref{fig:adv_dep}, even with i.i.d departures. Fix $n \geq 1$ and assume that departures are distributed according to the following distribution: w.p. $\nicefrac{1}{n}$, $d_i = n^2$, and w.p. $(1 - \nicefrac{1}{n})$, $d_i = 0$.

  The arrivals are defined as follows: the first $n \ln{n}$ vertices have no edge between themselves. The adversary then selects $K \in [0, \sqrt{n}]$.
  For $i \leq n \ln{n}$ and $j \in [n \ln{n}, n \ln{n} + K]$, $v_{i,j} = M^j$. Where $M$ is a large constant to be defined later. Vertices $j > n \ln{n} + K$ have no edges.

  Let $E_1$ be the event that there exists $j \in [n \ln{n} + 1, n\ln{n}+\sqrt{n}]$ such that $d_j > 1$.
  $$\P[E_1] = 1 - (1 - 1/n)^{\sqrt{n}} = \frac{1}{\sqrt{n}} + o\left(\nicefrac{1}{\sqrt{n}}\right).$$

  Let $E_2$ be the event that there are less than $\sqrt{n}$ vertices $j \in [0, n\ln{n}]$ such that $d_j > 1$. The (random) number of such vertices $X$ is binomially distributed with parameters $n \ln{n}$ and $\nicefrac{1}{n}$. Thus
  $$\P[E_2] = \P[X \leq \sqrt{n}] \geq 1 - O(\nicefrac{1}{\sqrt{n}}).$$

  We can write:
  $\E[\A] \leq \P[E_1 \cup E_2^c]\sum_{k = 0}^K M^k + \E[\A \mid E_1^c \cap E_2]$
  Conditional on $E_1^c$ and $E_2$, the best any algorithm can do is match each vertex $j \in [n\ln{n}+1, n\ln{n}+ \sqrt{n}]$ with probability $\ln{n} / \sqrt{n}$.
  Therefore $\E[\A] \leq O(\nicefrac{\ln{n}}{\sqrt{n}}) \sum_{k = 0}^K M^k$.

  Let $E_3$ be the event that there exists $i \in [0, n\ln{n}]$ such that $d_i > 1$. $\P[E_3] \geq (1 - \frac{1}{n})$. Therefore, $\E[\mathcal{O}] \geq M^k \P[E_3] \geq (1 - \frac{1}{n}) M^k$.
  For M large enough, we can conclude that $\nicefrac{\E[\A]}{\E[\mathcal{O}]} = O(\nicefrac{1}{\sqrt{n}})$.

\end{proof}

Finally, we consider the \emph{Stochastic Unknown Departures} (SUD) setting where the adversary chooses a departure rate $\delta$, and departures $d_i$ are i.i.d geometric random variables with parameter $\delta$. The online  algorithm knows $\delta$ but does not know $d_i$ even when $i$ becomes critical.

\begin{claim}
  Even when the departure process $\mathcal{D}$ is memoryless, if the algorithm doesn't know when vertices become critical, it cannot obtain a constant competitive ratio.
\end{claim}

\begin{proof}
  Consider the graph in Figure \ref{fig:adv_dep}, and assume that at each time step, an unmatched vertex in the graph has probability $1 - \delta$ of departing.

  Conditional on vertex $1$ being present at time $k$, let $x_k$ be the probability that the algorithm matches $1$ to $k$. We have: $\A = \sum_{k = 2}^K x_k \delta^k M^k$.
  Furthermore, observe that $\sum_{k = 2}^n x_k \leq 1$. Therefore there exists $l$ such that $x_l \leq 1/n$. Then take $K = l$.
  $$\A \leq x_{l} \delta^{l} M^{l} + \delta^{l + 1} M^l + \sum_{k \leq l - 1} \delta^{k} M^{k} \leq \mathcal{O} \left(x_{l} + \delta + \sum_{k
  \leq l - 1} \delta^{k} M^{k - l}\right).$$
  Therefore  $\nicefrac{\A}{\mathcal{O}} \leq O(\nicefrac{1}{n})$ for $\delta$ small enough and $M$ large enough.
\end{proof}


==> main_result.tex <==
% !TEX root = adv_paper.tex

\section{Main results}

The example in Figure \ref{fig:hard:basic} illustrates a necessary condition for the algorithm to achieve a constant competitive ratio: with some probability, vertex $2$ needs to forgo the match with vertex $1$. In general, we ensure this property by assigning every vertex to be either a {\it seller} or a {\it buyer}.  Buyers may get matched at any time while sellers can match only once they become critical.


We will  first consider  the case in which the underlying graph is  bipartite, with buyers on one side and sellers on the other. To ensure that sellers never match before they become critical, we further assume that there is no edge between a seller $s$ and any buyer $b$ who arrived before $s$. Such a graph is called a {\it constrained} bipartite graph.

In Section \ref{sec:bipartite} we introduce an algorithm for the case in which  the input graph is constrained bipartite. Through a primal-dual analysis,  we establish that the algorithm achieves at least \nicefrac{1}{2} of the offline total reward.

In Section \ref{sec:arbitrary} we consider  arbitrary graphs. For such graphs, we artificially generate a two-sided market by creating a buyer and a seller copy of each vertex. The matching produced by the algorithm in this  bipartite graph, is then transformed into a matching in the original graph by a carefully constructed randomized process. This process loses an additional factor of $2$.

\subsection{Algorithm for constrained bipartite graphs}
\label{sec:bipartite}

We assume here that the input is a constrained bipartite graph. Vertices on one side are called {\it buyers} and vertices on the other side are called  {\it sellers}, and there is no edge between a buyer $b$ and a seller $s$ if $b$ arrives before $s$ ($b<s$).

Note that even in this simplified setting no online algorithm can find the optimum solution. This is because when a new buyer arrives, she may create an augmenting path in the offline graph in which some of the vertices are already departed. We describe this in more details in  Claim \ref{cl:ex:bipartite_constrained}.

We  introduce the Dynamic Deferred Acceptance (DDA) algorithm, which takes as input a constrained bipartite graph and returns a matching.
The main idea is to maintain a temporary maximum-weight matching $m$ at all times during the run of the algorithm. This matching is updated according to an auction mechanism: every seller $s$ is associated with a \emph{price} $p_s$, which is initiated at zero upon arrival. Every  buyer $b$ that is present in the market is associated with a \emph{profit margin} $q_b$ which corresponds to the value of matching to their most prefered seller minus the price associated with that seller.
Every time a new buyer joins the market, she bids on her most prefered seller at the current set of prices. This triggers a bidding process that terminates when no unmatched buyer can profitably bid on a seller.

A tentative match between a buyer and a seller is converted into a real match only if the seller is critical, i.e. she has been present for $d$ time periods and is about to depart. At that time, both the seller and the buyer to whom she is matched depart from the market. This ensures that sellers never get matched before they become critical. If a buyer becomes critical we let her depart unmatched.

\begin{algorithm}[H]
  \caption{The Dynamic Deferred Acceptance algorithm}\label{alg:DDA}
  \begin{itemize}
  \item At any point $t$ during the algorithm, maintain a set of sellers $S_t$, a set of buyers $B_t$, as well as a matching $m$, a price $p_s$ for every seller $s \in S_t$, and a marginal profit $q_b$ for every buyer $b \in B_t$.
  \item Process each event in the following way:
  \begin{enumerate}
    \item\label{step:arrival:seller}\emph{Arrival of a seller s:} Initialize $p_s \leftarrow0$ and $m(s) \leftarrow \emptyset$.
    \item\label{step:arrival:buyer}\emph{Arrival of a buyer $b$:} Start the following {\em ascending auction.} \\
    Repeat
      \begin{enumerate}
         \item Let $q_b \leftarrow \max_{s' \in S_t} v_{s', b} - p_{s'}$ and $s \leftarrow \argmax_{s' \in S_t} v_{s', b} - p_{s'}$.
         \item If $q_b > 0$ then
         \begin{enumerate}
         \item $p_s \leftarrow p_s+\epsilon$.
         \item $m(s)\leftarrow b$ (tentatively match $s$ to $b$)
         \item Set $b$ to $\emptyset$ if $s$ was not matched before. Otherwise, let $b$ be the previous match of $s$.
    	\end{enumerate}
    \end{enumerate}
    Until $q_b \leq 0$ or $b = \emptyset$.
    \item\label{step:departure:seller} \emph{Departure of a seller s:} If seller $s$ becomes critical and  $m(s) \neq \emptyset$, finalize the matching of $s$ and $m(s)$ and collect the reward of $v_{s, m(s)}$.

  \end{enumerate}
\end{itemize}
\end{algorithm}

The ascending auction phase  in our algorithm is similar to the auction algorithm by \cite{bertsekas1988auction}. Prices (for overdemanded sellers) in this auction increase by  $\epsilon$ to ensure termination, and optimality is proven  through $\epsilon$-complementary slackness conditions. For the simplicity of exposition we presented the auction algorithm but for the analysis, we consider the limit $\epsilon \rightarrow 0$ and assume the auction phase terminates with the maximum weight matching. Another way to update the matching is through the  Hungarian algorithm \cite{kuhn1955hungarian}, where  prices are increased simultaneously along an alternating path that only uses edges for which the dual constraint is tight.

The auction phase is always initiated at the existing  prices and profit margins. This, together with the fact that the graph is bipartite, ensures that prices never decrease and and marginal profits never increase throughout the algorithm. Furthermore, the prices and marginal profits of the vertices that are present in the market form an optimum dual for the matching linear program (see Appendix \ref{app:missing_proofs} for more details).
\begin{lemma}
\label{lem:mon}
Consider the DDA algorithm on a constrained bipartite graph.
\begin{enumerate}
\item Throughout the algorithm,  prices corresponding the sellers never decrease and the profit margins of buyers never increase.
\item At the end of every ascending auction,  prices of the sellers and the marginal profits of the buyers form an optimal solution to the dual  of the matching linear program associated with  buyers and sellers present at that particular time.
\end{enumerate}
\end{lemma}

Maintaining a  maximum-weight matching along with optimum dual variables does not guarantee an efficient matching for the whole graph. The dual values are not always feasible for the offline problem. Indeed, the profit margin of some  buyer $b$ may  decrease after some seller departs the market. This is because $b$ may face increasing competition from new buyers, while the bidding process excludes sellers that have already departed the market (whether matched or not).

\begin{proposition}
  \label{prop:factor2}
  DDA is $\nicefrac{1}{2}$-competitive for constrained bipartite  graphs.
\end{proposition}

The proof, given in Section \ref{sec:analysis}, relies on a primal-dual argument. For any arriving buyer $b$ we denote by $q_b^i$ her \emph{initial profit margin} after the ascending auction %(step \ref{step:ascending})
terminates.  When a buyer $b$ is matched or departs, we set $q_{b}^f$ to be her \emph{final profit margin} at that time. Similarly when a seller $s$ departs or is matched, we denote by $p_s^f$ her \emph{final price} at that time.

The proof of the proposition relies on the following three ingredients. First, letting  $S = \cup_{t \in [1,T]} S_t$ and $B = \cup_{t \in [1,T]} B_t$, then the algorithm collects
$$\sum_{s \in S} v_{s, m(s)} = \sum_{s \in S} p_s^f + \sum_{b \in B} q_b^f.$$
Second, although the  final dual variables $(p^f, q^f)$ are not dual feasible, the pair $(p^f, q^i)$ is a feasible dual solution of the offline matching problem.
Finally, we  obtain a  factor $2$ by observing that  $$\sum_{s\in S} p_s^f + \sum_{b \in B} q_b^f = \sum_{b \in B} q_b^i.$$

\subsection{Arbitrary graphs}
\label{sec:arbitrary}

In the previous section, we constructed an algorithm for constrained bipartite graphs, we now extend it to arbitrary graphs.

A naive way to generate a constrained bipartite graph from an arbitrary one is to randomly assign each vertex to be  either a seller or a buyer, independently and with probability \nicefrac{1}{2}. Then we remove any edge between each seller and buyers who have arrived before her. This approach yields the {\it Simple Dynamic Deferred Acceptance} (SDDA) algorithm:

\begin{algorithm}
\caption{Simple Dynamic Deferred Acceptance (SDDA)}
\begin{itemize}
\item For each vertex $t=1,\ldots, T$:
\begin{enumerate}
\item[]  Toss a fair coin to decide whether $t$ is a  \emph{seller} or a \emph{buyer}. Construct the corresponding constrained bipartite graph by keeping only the edges between each buyer and the sellers who arrived at most $d$ steps before her.
\end{enumerate}
\item Run the DDA algorithm on the resulting constrained bipartite graph.
\end{itemize}
\end{algorithm}

\begin{corollary}
  \label{cor:factor8}
  SDDA is $\nicefrac{1}{8}$-competitive for arbitrary graphs.
\end{corollary}

Observe that for $i < j$, edge $(i,j)$ in the original graph remains in the generated bipartite graph with probability $1/4$ (if $i$ is a seller and $j$ is a buyer). We then use proposition \ref{prop:factor2} to prove that SDDA is $\nicefrac{1}{8}$-competitive.

One source of inefficiency in SDDA is that the decision whether an agent is a seller or a buyer is done independently at random and without taking the graph structure into consideration. We next introduce  the   {\it Postponed Dynamic Deferred Acceptance} algorithm that postpones these decisions for as long as possible to enable a more careful construction of the constrained bipartite graph.

When a vertex $k$ arrives, we add two copies of $k$ to an virtual graph: first a seller $s_k$ and then a buyer $b_k$. Seller $s_k$ initially does not have any edges, and buyer $b_k$ has edges towards any vertex $s_l \in S_k$ with value $v_{l,k}$. Then we run the DDA algorithm with the virtual graph as input. When  a vertex $k$ becomes critical, $s_k$ and $b_k$ successively become critical in the virtual graph, and we compute their matches generated by $DDA$.

Both $s_k$ and $b_k$ can be matched in this process.  If we were to honor both matches, the outcome would correspond to a 2-matching, in which each vertex has degree at most 2. Now observe that because of the structure of the constrained bipartite graph, this 2-matching does not have any cycles; it is just a collection of disjoint paths. We decompose each path into two disjoint matchings and choose each matching with probability  $1/2$.

In order to do that, the algorithm must determine, for each original vertex $k$, whether the virtual buyer $b_k$ or virtual seller $s_k$ will be used in the final matching. We will say that $k$ is a \emph{buyer} or \emph{seller} depending on which copy is used. We say that vertex $k$ is \emph{undetermined} when the algorithm has not yet determined which virtual vertex will be used. When an undetermined vertex becomes critical, the algorithm  flips a fair coin to decide whether to match according to the buyer or seller copy. This decision is then propagated to the next vertex in the 2-matching: if $k$ is a \emph{seller} then the next vertex will be a \emph{buyer} and vice-versa.
That ensures that assignments are correlated and saves a factor $2$ compared to uncorrelated assignments in \emph{SDDA}.

\begin{algorithm}[ht]
\caption{Postponed Dynamic Deferred Acceptance (PDDA)}
\label{alg:QDDA}
\begin{itemize}
\item At any point $t$ during the algorithm, maintain an virtual bipartite graph between a set of sellers $S_t$ and a set of buyers $B_t$. Also maintain a matching $m$, a price $p_s$ for every virtual seller $s \in S_t$, and a marginal profit $q_b$ for every virtual buyer $b \in B_t$.
For each (real) vertex $k$, maintain $k$'s status as either \emph{undetermined}, \emph{buyer} or \emph{seller}.

\item Process each event in the following way:
\begin{enumerate}
  \item \emph{Arrival of a vertex $k$:}
  \begin{enumerate}
  	\item Set $k$'s status to be \emph{undetermined}.
    \item \emph{Add a virtual seller:} $S_t \leftarrow S_{t} \cup \{s_k\}$ and $p_{s_k} \leftarrow 0$.
    \item \emph{Add a virtual buyer:} $B_t \leftarrow B_{t} \cup \{b_k\}$ and $q_{b_k} \leftarrow \max_{s \in S_t} v_{s, b_k} - p_s$.
    If $q_{b_k}>0$, start an ascending auction in DDA, and update $m$, $p$, $q$ accordingly.
  \end{enumerate}
  \item \emph{Vertex $k$ becomes critical:}
  \begin{enumerate}
    \item Let $l$ be such that $m(s_k)= b_l$.
Set $B_t \leftarrow B_t \setminus \{b_k\}$, $S_t \leftarrow S_t \setminus \{s_k\}$, and $B_t \leftarrow B_t \setminus \{b_l\}$. (\emph{match in the virtual graph.}) %($s_l$ stays in $S_t$.)
    \item If $k$'s status is \emph{undetermined}, w.p $\nicefrac{1}{2}$ set it to be either \emph{seller} or \emph{buyer}.
    \begin{enumerate}
      \item\label{step:seller}\emph{If $k$ is a seller:} finalize the matching of $k$ to $l$ and collect the reward $v_{k,l}$. If $l \neq \emptyset$, set $l$ to be a buyer.
      \item\label{step:buyer}\emph{If $k$ is a buyer:} If $l \neq \emptyset$, set $l$ to be a seller.
    \end{enumerate}
  \end{enumerate}
\end{enumerate}
\end{itemize}
\end{algorithm}

\begin{theorem}
  \label{th:factor4}
  PDDA is $\nicefrac{1}{4}$-competitive.
\end{theorem}

\noindent
The proof of Theorem \ref{th:factor4} is deferred to Section \ref{sec:analysis}. It relies on the following three ingredients.
First, the algorithm collects $$\E\left[\sum_{k \in S} p_{s_k}^f + \sum_{l \in B} q_{b_l}^f\right] = \frac{1}{2} \left(\sum_{k \in [1, T]} p_{s_k}^f + \sum_{l \in [1, T]} q_{b_l}^f\right),$$ where the expectation is taken over the random assignments of \emph{undetermined} vertices to be sellers or buyers.
Second, $(p_{s_k}^f + q_{b_k}^i)_{k \in [1, T]}$ is a feasible dual solution of the offline matching problem. Finally,  similar  to the proof of \ref{prop:factor2}, we use the following equality: $$\sum_{k \in [1, T]} p_{s_k}^f + \sum_{l \in [1, T]} q_{b_l}^f = \sum_{l \in [1, T]} q_{b_l}^i.$$


==> numerical.tex <==
% !TEX root = adv_paper.tex

\section{Numerical results}
In \emph{PDDA}, we compute a 2-matching over the vertices that are currently present, and select each edge with probability $\nicefrac{1}{2}$. Although this randomization is useful to hedge against the worst case instance, it may be ineffective when the compatibility graph is not generated by an adversary.

Nonetheless, some of the key ideas behind \emph{PDDA} may be useful to construct algorithms that perform well on non-adversarial graphs. This motivates a modified version of the Dynamic Defered Dcceptance algorithm, termed \emph{MDDA}, in which vertices are no longer separated into buyers and sellers and every vertex now has a \emph{price}.

Under MDDA, prices are reset to $0$ after each arrival, and  an auction is conducted on the non-bipartite graph: while there exists an unmatched vertex, one is selected  at random and it bids on its most prefered match. This leads to a tentative matching $M$ over all the vertices that are currently present in the graph\footnote{Note that because the graph is non-bipartite, this auction mechanism may fail to converge to a maximum-weight matching.}.  When a vertex becomes critical, it is matched  according to the tentative matching $M$. This modified algorithm does not have theoretical guarantees, but we will show that it performs well on data-driven compatibility graphs.

Note that MDDA can be thought of as a re-optimization algorithm, where the optimal matching is re-computed when new information becomes available. One can replace the auction mechanism with any algorithm that computes a maximum-weight matching. We implemented this algorithm, termed here \emph{Re-Opt}, where the matching is found by solving a mixed-integer program at each time step.

We  compare the MDDA and Re-Opt  algorithms against three benchmarks that have been previously consdiered, or that are commonly used in practice:
\begin{itemize}
  \item[-] The \emph{Greedy} algorithm. The algorithm  matches vertices as soon as possible to their available neighbor with the highest value (ties are broken in favor of the earliest arrival).
  \item[-] The \emph{Batching}($k$) algorithm. The algorithm waits $k$ times-steps  and then finds a maximum-weight matching. Unmatched vertices are kept in the next batch.\footnote{See \cite{agatz2011dynamic,ashlagi2013kidney} in the case of ride-sharing and kidney exchange respectively.} We  report the best simulation results across parameters $k = 5, 10, 50, 100, 200, 300$.
  \item[-] The Patient algorithm. This algorithm waits until waits until a vertex becomes critical, and matches it to the neighbor with the highest  match value (ties are broken in favor of the earliest arrival). This allows to seperate the value from  knowing the time in which vertices become  critical and the value of optimization.
\end{itemize}

\subsection*{Data}

The first experiment uses data from the National Kidney Registry (NKR), which consists of 1681 patient-donor pairs who have joined the NKR. For any two patient-donor pairs $k$ and $t$, we can determine whether the patient from each pair would have been medically eligible to receive the kidney from the other pair's donor, had they had been present at the same time. If that is the case, we set $v_{k,l} = 1$, otherwise  and $v_{k,l} =0$ (in particular we simply try to maximize the number of matches)\footnote{We ignore here the possibility of larger cyclic exchanges (3 or 4-cycles) or chains, which are common in practice.}.

In the second instance, we use New York City yellow cabs dataset \footnote{http://www.andresmh.com/nyctaxitrips/}, which consists of rides taken in NYC over a year. For any pair $k,l$ of trips, we can compute the Euclidian distance that would have been traveled had the two passengers taken the same taxi (with multiple stops). The value $v_{k,l}$ represents the ``distance saved'' by combining the trips.

In both cases, this enables us to generate a dynamic graph in the following way. For $t \in [1,T]$:
\begin{enumerate}
 \item Sample with replacement an arrival $t$ from the dataset.
 \item For any vertex $l$ that is present in the pool, compute the value $v_{t,l}$ of matching $t$ to $l$.
 \item Sample a departure time $d_t \sim \mathcal{D}$.
\end{enumerate}

We  consider two settings, termed \emph{deterministic} and \emph{stochastic} respectively, in which $\mathcal{D}$ is either constant with value $d$, or exponentially distributed with mean $d$. We will report simulation results for $d = 50, 100, 200, 300$.

\subsection*{Results}

In Figure \ref{fig:taxi}, we observe that both the \emph{Patient} and \emph{Batching} algorithms outperform \emph{Greedy}. Intuitively, having vertices wait until they become critical helps to thicken the market and gives vertices higher valued match options. We notice that when departures are deterministic, \emph{Batching} with the optimal batch size will be almost as efficient as \emph{Re-Opt}. However when the departures are stochastic, there is value in matching vertices as they become critical (\emph{MDDA} and \emph{Re-Opt}).

\begin{figure}[ht!]
  \centering
\includegraphics[scale=0.34]{figs/taxi_deterministic.pdf}
\hspace{0.2cm}
\includegraphics[scale=0.34]{figs/taxi_stochastic.pdf}
\caption{Performance of our 4 algorithms on taxi data (weighted compatibility graph).}
\label{fig:taxi}
\end{figure}

Figure \ref{fig:kidney} provides the results for the kidney exchange simulations. In this case, the compatibility graph is unweighted, which implies that because we break ties in favor of the earliest arrival and departures are in order of arrival, \emph{Greedy} and \emph{Patient} are equivalent. Again, \emph{Batching} performs relatively well in the deterministic case (if $b<d$,  no vertex will depart before it is included in one batch), but very poorly in the stochastic case. %In contrast, \emph{MDDA} and \emph{Re-Opt} perform well in both situations.

\begin{figure}[ht!]
  \centering
\includegraphics[scale=0.33]{figs/kidney_deterministic.pdf}
\hspace{0.2cm}
\includegraphics[scale=0.33]{figs/kidney_stochastic.pdf}
\caption{Performance of our 4 algorithms on kidney data (unweighted compatibility graph).}
\label{fig:kidney}
\end{figure}

In both datasets, we observe that \emph{Re-Opt} outperforms all other algorithm, although in the cases where the departures are deterministic, \emph{Batching} performs close to \emph{Re-Opt} when the batch size $k$ is carefully chosen.  This shows the value of both having information on agents' departure times and also  subsequent optimization.

It is important to note that the experiments we ran do not take into account the cost of waiting. We think that a richer model that accounts for this would be an interesting future direction.
Two interesting areas for future work include the setting when the information about agent's departure times is uncertain, as well as models that are less restrictive than the adversarial setting (see, e.g., \citet{ozkan2016dynamic}).

